HOSS!

The Hall-D Online Skim System (HOSS) was developed to simultaneously solve two issues for the high intensity GlueX experiment. One was to parallelize the writing of raw data files to disk in order to improve bandwidth. The other was to distribute the raw data across multiple compute nodes in order to produce calibration \textit{skims} of the data online. The highly configurable system employs RDMA, RAM disks, and zeroMQ driven by Python to simultaneously store and process the full high intensity GlueX data stream.

==> hoss_RAID+DB_gen16.config.tex <==
#
# This configuration will only run the first stage of skimming
# so that the DB can be updated with the trigger counts. It
# will not generate final skim files.
#
#-----------------------------------------------------------------
#
# This is a configuration file for the hd_data_flow.py script.
#
# Syntax is as follows:
#
# Sections start with either "stage:" or "distribute:".
#
# "stage:" sections describe directories where files should be
# linked to once they are no longer being written to. Each file
# may appear in multiple destinations. Once a file is linked in
# all of the specified directories, the original is unlinked.
# Directories specified in stage sections must be local (i.e.
# not prefixed with a host name.)
#
# "distribute:" sections describe directories that files should
# be moved to using a round-robin algorithm. Each file appears
# in only one of the destinations. Destinations may be either
# local or remote and a mixture of both types is allowed.
#
#  Both section types support multiple "source" lines and 
# multiple "destination" lines. The source lines may contain
# wildcards and any syntax supported by python's glob.glob().
# The destination lines must specify a directory (no wildcards).
# 
# For the "stage:" sections all sources and destinations must
# be on the same filesystem.
#
# For "distribute:" sections, the destinations may indicate a
# remote host by specifying it with a colon (:) in front of
# the destination directory. "destination" lines that specify
# a host will have the files copied using hdrdmacp. Ones that
# do not specify a host will copy the files using rsync. Both
# types may be mixed in the same section if you want to copy 
# some files to a local disk and send some to a remote host.
#
#

# Uncomment to turn on test mode. (See comments in TESTING section below)
#TESTMODE:


#-------------------------------------------------------------------
# Misc Config
#
# Set misc. config parameters.
#
# ALIAS:        Define an alias. This allows a shorthand to be used in the rest
#               of this file where groups of nodes may be referenced with %ALIASNAME.               
#
# MAX_PROCS:    Set maximum number of processes allowed to run simultaneously on a host
#
# FILE_TIMEOUT: Sets a maximum time since last access before a file is deleted.
#               First argument is in seconds. Second argument is directory to start in.
#               Files in the specified directory and any subdirectories are subject
#               to deletion. Third argument are nodes on which to apply this rule.
#
# ALARM:        Set alarm threshold for free disk space.
#
# DB_HOST:      The DB_X: options specify connection info for a MySQL DB to insert
# DB_USER:      file movement information into. 
# DB_PASS:
# DB_DATABASE:
# DB_NODES:     DB_NODES: lists the nodes which should make entries into the DB

ALIAS:   RAID_NODES        gluonraid3,gluonraid4,gluonraid5
ALIAS: MASTER_NODES        gluondaqbuff,%RAID_NODES
ALIAS: WORKER_NODES_RAID3  gluon112,gluon113
ALIAS: WORKER_NODES_RAID4  gluon114,gluon115
ALIAS: WORKER_NODES_RAID5  gluon116,gluon117
ALIAS: WORKER_NODES        %WORKER_NODES_RAID3,%WORKER_NODES_RAID4,%WORKER_NODES_RAID5

MAX_PROCS: 2 %WORKER_NODES
MAX_PROCS: 4 %MASTER_NODES

FILE_TIMEOUT: 200 /media/ramdisk/@TESTDIR/ %WORKER_NODES

ALARM: 30GB /media/ramdisk %MASTER_NODES
ALARM:  1GB /media/ramdisk %WORKER_NODES

DB_HOST:      gluondb1.jlab.org
DB_USER:      hoss
DB_PASS:    
DB_DATABASE:  HOSS
DB_NODES:     %MASTER_NODES


#-------------------------------------------------------------------
# TESTING
# The following is used for testing. To turn on test mode, uncomment
# the line with TESTMODE: at the top of this file.
# Note that these directories are hardwired to include the TEST
# directory so that the they don't accidentally delete files 
# from the actual directories holding real data when TESTMODE is
# turned off. By uncommenting the TESTMODE: line, all instances
# of @TESTDIR/ in this file will be replaced by TEST. Otherwise,
# they are replaced by an empty string.
#
# The REMOVETREE: line below will cause all directories and files
# from the specified directory to be removed before starting the
# scans. This is intended for testing as a way to clear out the
# ram disks.
#
# Similar to above, the KILLALL: line will cause the specified 
# process to be killing (permissions permitting). This is intended
# to clear out lingering processes at startup.
#
KILLALL:    hd_ana               %WORKER_NODES
KILLALL:    hdskims              %WORKER_NODES
KILLALL:    hdmk_skims.py        %WORKER_NODES
REMOVETREE: /media/ramdisk/TEST  %MASTER_NODES,%WORKER_NODES
REMOVETREE: /data1/TEST          %MASTER_NODES,%WORKER_NODES
REMOVETREE: /data2/TEST          %MASTER_NODES,%WORKER_NODES
REMOVETREE: /data3/TEST          %MASTER_NODES,%WORKER_NODES
REMOVETREE: /data4/TEST          %MASTER_NODES,%WORKER_NODES


stage: %RAID_NODES
	
	# Raw data files in both the staged_for_tape directory and volatile directories
	source      /data*/TEST/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run*/*.evio
	source      /data*/TEST/rawdata/volatile/@RUNPERIOD/rawdata/Run*/*.evio

	# Skim files in both the staged_for_tape directory and volatile directories
	source      /data*/TEST/calib/staged_for_tape/@RUNPERIOD/calib/ver00/*/Run*/*.*
	source      /data*/TEST/calib/volatile/@RUNPERIOD/calib/ver00/*/Run*/*.*

 	# Delete files
	destination /dev/null


#-------------------------------------------------------------------
# DAQ
#
# Copy from buffer disk to RAM disk on RAIDs
#
# note: Two source directories are specified, but CODA currently
#       only writes to the long ones.
#       Also, CODA may be configured to use either gluondaqbuff 
#       or a gluonraid RAM disk for writing.
#
#- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
#
# This section defines the fall-back configuration where the DAQ writes
# directly to a RAID partition. It looks in /data*/rawdata/active/...
# for evio files and copies them to both volatile and staged_for_tape
# directories. Files are NOT copied to any other computer and no
# processing is done.


stage: gluonraid3,gluonraid4,gluonraid5
	source /data1/@TESTDIR/rawdata/active/RunPeriod-2019-11/rawdata/Run07*/*.evio
	destination /data1/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data1/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER
stage: gluonraid3,gluonraid4,gluonraid5
	source /data2/@TESTDIR/rawdata/active/RunPeriod-2019-11/rawdata/Run07*/*.evio
	destination /data2/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data2/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER
stage: gluonraid3,gluonraid4,gluonraid5
	source /data3/@TESTDIR/rawdata/active/RunPeriod-2019-11/rawdata/Run07*/*.evio
	destination /data3/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data3/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER
stage: gluonraid3,gluonraid4,gluonraid5
	source /data4/@TESTDIR/rawdata/active/RunPeriod-2019-11/rawdata/Run07*/*.evio
	destination /data4/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data4/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER

#- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
#
# This section implements copying of files from gluondaqbuff to the
# raid disks, but also to the farm nodes for processing.
#

stage: gluondaqbuff
   source      /media/ramdisk/@TESTDIR/active/*.evio
	source      /media/ramdisk/@TESTDIR/active/rawdata/active/RunPeriod-*/rawdata/Run*/*.evio
	destination /media/ramdisk/@TESTDIR/rawdata_in

distribute: gluondaqbuff
   source      /media/ramdisk/@TESTDIR/rawdata_in/*.evio
   destination gluonraid3:/media/ramdisk/@TESTDIR/active
   destination gluonraid4:/media/ramdisk/@TESTDIR/active
   destination gluonraid5:/media/ramdisk/@TESTDIR/active

stage: %RAID_NODES
   source      /media/ramdisk/@TESTDIR/active/*.evio
	source      /media/ramdisk/@TESTDIR/active/rawdata/active/RunPeriod-*/rawdata/Run*/*.evio
   destination /media/ramdisk/@TESTDIR/rawdata_staged_for_disk
   destination /media/ramdisk/@TESTDIR/rawdata_staged_for_skim


#-------------------------------------------------------------------
# RAWDATA
#
# First copy from ramdisk to one of the RAID partitions and then
# make links in staged_for_tape and volatile directories.

distribute: %RAID_NODES
   source      /media/ramdisk/@TESTDIR/rawdata_staged_for_disk/*.evio
	destination /data1/@TESTDIR/rawdata/staged_for_disk
	destination /data2/@TESTDIR/rawdata/staged_for_disk
	destination /data3/@TESTDIR/rawdata/staged_for_disk
	destination /data4/@TESTDIR/rawdata/staged_for_disk

stage: %RAID_NODES
   source      /data1/@TESTDIR/rawdata/staged_for_disk/*.evio
	destination /data1/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data1/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER
stage: %RAID_NODES
   source      /data2/@TESTDIR/rawdata/staged_for_disk/*.evio
	destination /data2/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data2/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER
stage: %RAID_NODES
   source      /data3/@TESTDIR/rawdata/staged_for_disk/*.evio
	destination /data3/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data3/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER
stage: %RAID_NODES
   source      /data4/@TESTDIR/rawdata/staged_for_disk/*.evio
	destination /data4/@TESTDIR/rawdata/staged_for_tape/@RUNPERIOD/rawdata/Run@RUNNUMBER
	destination /data4/@TESTDIR/rawdata/volatile/@RUNPERIOD/rawdata/Run@RUNNUMBER

#-------------------------------------------------------------------
# SKIMS
#
# - Copy to farm node
# - Run hdmk_skims.py in trigger count only mode on farm node and enter into DB
#

# Clear out files from (potentially) non-test directories
# WARNING: If there are files lingering on worker nodes awaiting
# processing, this will delete them!
REMOVETREE: /media/ramdisk/@TESTDIR/active                    %WORKER_NODES
REMOVETREE: /media/ramdisk/@TESTDIR/rawdata_staged_for_skim   %WORKER_NODES,%MASTER_NODES
REMOVETREE: /media/ramdisk/@TESTDIR/skim_out                  %WORKER_NODES,%MASTER_NODES

distribute: gluonraid3
   source      /media/ramdisk/@TESTDIR/rawdata_staged_for_skim/*.evio
	destination %WORKER_NODES_RAID3:/media/ramdisk/@TESTDIR/active

distribute: gluonraid4
   source      /media/ramdisk/@TESTDIR/rawdata_staged_for_skim/*.evio
	destination %WORKER_NODES_RAID4:/media/ramdisk/@TESTDIR/active

distribute: gluonraid5
   source      /media/ramdisk/@TESTDIR/rawdata_staged_for_skim/*.evio
	destination %WORKER_NODES_RAID5:/media/ramdisk/@TESTDIR/active

# n.b. use stage section to ensure only complete files appear in rawdata_staged_for_skim
stage:      %WORKER_NODES
   source      /media/ramdisk/@TESTDIR/active/*.evio
	destination /media/ramdisk/@TESTDIR/rawdata_staged_for_skim

# The "process_out" line declares the output directory for the process so HOSS can kill the
# process if the output disk fills up
distribute: %WORKER_NODES
   source      /media/ramdisk/@TESTDIR/rawdata_staged_for_skim/*.evio
   process     hdlog hdmk_skims.py -d -c @INFILE /media/ramdisk/@TESTDIR/skim_out
	process_out /media/ramdisk/@TESTDIR/skim_out





